Money, Time, and Grant Design

The design of research grants has been hypothesized to be a useful tool for influencing researchers and their science. We test this by conducting two thought experiments in a nationally representative survey of academic researchers. First, we offer participants a hypothetical grant with randomized attributes and ask how the grant would influence their research strategy. Longer grants increase researchers' willingness to take risks, but only among tenured professors, which suggests that job security and grant duration are complements. Both longer and larger grants reduce researchers' focus on speed, which suggests a significant amount of racing in science is in pursuit of resources. But along these and other strategic dimensions, the effect of grant design is small. Second, we identify researchers' indifference between the two grant design parameters and find they are very unwilling to trade off the amount of funding a grant provides in order to extend the duration of the grant $\unicode{x2014}$ money is much more valuable than time. Heterogeneity in this preference can be explained with a straightforward model of researchers' utility. Overall, our results suggest that the design of research grants is more relevant to selection effects on the composition of researchers pursuing funding, as opposed to having large treatment effects on the strategies of researchers that receive funding.

==> figtab/stub_capeomnibustesthet_accur_len_xp1.tex <==
=0.423


==> figtab/stub_capeomnibustesthet_accur_len_xp2.tex <==
=0.350


==> figtab/stub_capeomnibustesthet_accur_siz_xp1.tex <==
=0.866


==> figtab/stub_capeomnibustesthet_accur_siz_xp2.tex <==
=0.960


==> figtab/stub_capeomnibustesthet_newdi_len_xp1.tex <==
=0.529


==> figtab/stub_capeomnibustesthet_newdi_len_xp2.tex <==
=0.314


==> figtab/stub_capeomnibustesthet_newdi_siz_xp2.tex <==
$<$0.001


==> figtab/stub_capeomnibustesthet_riski_len_xp2.tex <==
=0.001


==> figtab/stub_capeomnibustesthet_riski_siz_xp1.tex <==
=1.000


==> figtab/stub_capeomnibustesthet_riski_siz_xp2.tex <==
=0.989


==> figtab/stub_capeomnibustesthet_sizeo_len_xp1.tex <==
=1.000


==> figtab/stub_capeomnibustesthet_sizeo_len_xp2.tex <==
=1.000


==> figtab/stub_capeomnibustesthet_sizeo_siz_xp1.tex <==
=1.000


==> figtab/stub_capeomnibustesthet_sizeo_siz_xp2.tex <==
=1.000


==> figtab/stub_capeomnibustesthet_speed_len_xp1.tex <==
=1.000


==> figtab/stub_capeomnibustesthet_speed_len_xp2.tex <==
=1.000


==> figtab/stub_capeomnibustesthet_speed_siz_xp1.tex <==
=0.992


==> figtab/stub_capeomnibustesthet_speed_siz_xp2.tex <==
=1.000


==> figtab/tab_capeblpunivar_accur_xp2.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}

\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\newcolumntype{L}{>{\raggedright\arraybackslash}X}
\newcolumntype{C}{>{\centering\arraybackslash}X}

\begin{tabular}{lc}

\hline \hline
& Univar. \\ 
 & coef. \\ 
\hline \\
\underline{\emph{Size}}& \\
\emph{n/a}& \\
& \\
\underline{\emph{Duration}}& \\
\emph{n/a}& \\
\\ \hline \hline 

\end{tabular}

}


==> figtab/tab_capeblpunivar_newdi_xp2.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}

\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\newcolumntype{L}{>{\raggedright\arraybackslash}X}
\newcolumntype{C}{>{\centering\arraybackslash}X}

\begin{tabular}{lc}

\hline \hline
& Univar. \\ 
 & coef. \\ 
\hline \\
\underline{\emph{Size}}& \\
[0.5em]Outputs: Books&0.021\sym{***} \\
& \\
\underline{\emph{Duration}}& \\
\emph{n/a}& \\
\\ \hline \hline 

\end{tabular}

}


==> figtab/tab_capeblpunivar_riski_xp2.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}

\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\newcolumntype{L}{>{\raggedright\arraybackslash}X}
\newcolumntype{C}{>{\centering\arraybackslash}X}

\begin{tabular}{lc}

\hline \hline
& Univar. \\ 
 & coef. \\ 
\hline \\
\underline{\emph{Size}}& \\
\emph{n/a}& \\
& \\
\underline{\emph{Duration}}& \\
[0.5em]Tenured&0.085\sym{***} \\
[0.5em]Not on tenure-track&--0.099\sym{***} \\
\\ \hline \hline 

\end{tabular}

}


==> figtab/tab_capeblpunivar_sizeo_xp2.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}

\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\newcolumntype{L}{>{\raggedright\arraybackslash}X}
\newcolumntype{C}{>{\centering\arraybackslash}X}

\begin{tabular}{lc}

\hline \hline
& Univar. \\ 
 & coef. \\ 
\hline \\
\underline{\emph{Size}}& \\
[0.5em]Computer science&--0.171\sym{***} \\
& \\
\underline{\emph{Duration}}& \\
[0.5em]Outputs: Products&0.040\sym{***} \\
\\ \hline \hline 

\end{tabular}

}


==> figtab/tab_capeblpunivar_speed_xp2.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}

\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\newcolumntype{L}{>{\raggedright\arraybackslash}X}
\newcolumntype{C}{>{\centering\arraybackslash}X}

\begin{tabular}{lc}

\hline \hline
& Univar. \\ 
 & coef. \\ 
\hline \\
\underline{\emph{Size}}& \\
[0.5em]Outputs: Books&--0.021\sym{***} \\
[0.5em]Chemistry&--0.156\sym{***} \\
& \\
\underline{\emph{Duration}}& \\
\emph{n/a}& \\
\\ \hline \hline 

\end{tabular}

}


==> figtab/tab_gammarevisit.tex <==
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}         \\
\hline
            &                     \\
$\gamma_{\text{Not tenured}}$&       0.759\sym{***}\\
            &     (0.011)         \\
[0.5em]
            &                     \\
$\gamma_{\text{Tenured}}$&       0.773\sym{***}\\
            &     (0.009)         \\
[0.5em]
\hline
$ p$--value of diff.&        0.32         \\
$ N$ obs.   &       4,175         \\
\hline\hline
\end{tabular}


==> figtab/tab_grantinput_joint.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         \\
\hline
                    &                     &                     \\
Own salary          &                     &                     \\
[0.5em]
\hspace{3mm} $\times$ log(Duration)&      --0.049\sym{*}  &      --0.049\sym{*}  \\
                    &     (0.026)         &     (0.026)         \\
[0.5em]
\hspace{3mm} $\times$ log(Amount)&       0.056\sym{***}&       0.056\sym{***}\\
                    &     (0.014)         &     (0.014)         \\
[0.5em]
Training            &                     &                     \\
[0.5em]
\hspace{3mm} $\times$ log(Duration)&       0.005         &       0.005         \\
                    &     (0.040)         &     (0.040)         \\
[0.5em]
\hspace{3mm} $\times$ log(Amount)&       0.103\sym{***}&       0.103\sym{***}\\
                    &     (0.020)         &     (0.020)         \\
[0.5em]
Travel              &                     &                     \\
[0.5em]
\hspace{3mm} $\times$ log(Duration)&       0.015         &       0.015         \\
                    &     (0.021)         &     (0.021)         \\
[0.5em]
\hspace{3mm} $\times$ log(Amount)&      --0.004         &      --0.004         \\
                    &     (0.011)         &     (0.011)         \\
[0.5em]
Equip. or supplies  &                     &                     \\
[0.5em]
\hspace{3mm} $\times$ log(Duration)&      --0.006         &      --0.006         \\
                    &     (0.024)         &     (0.024)         \\
[0.5em]
\hspace{3mm} $\times$ log(Amount)&      --0.018         &      --0.018         \\
                    &     (0.012)         &     (0.012)         \\
[0.5em]
Others' salaries    &                     &                     \\
[0.5em]
\hspace{3mm} $\times$ log(Duration)&       0.024         &       0.024         \\
                    &     (0.019)         &     (0.019)         \\
[0.5em]
\hspace{3mm} $\times$ log(Amount)&      --0.055\sym{***}&      --0.055\sym{***}\\
                    &     (0.010)         &     (0.010)         \\
[0.5em]
\hline
$ L(\mathbf{X})$    &                     &           Y         \\
$ N i$ obs.         &       4,175         &       4,175         \\
$ N ij$ obs.        &      20,875         &      20,875         \\
\hline\hline
\end{tabular}
}


==> figtab/tab_grantstrat_all_lasso.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{9}{c}}
 \hline\hline
& & & & & & &Larger & & \\
 & &  &More & &New & &ongoing & &More \\
&Faster & &risk & &directions & &projects &  &accurate \\
                    &\multicolumn{1}{c}{(1)}         &            &\multicolumn{1}{c}{(2)}         &            &\multicolumn{1}{c}{(3)}         &            &\multicolumn{1}{c}{(4)}         &            &\multicolumn{1}{c}{(5)}         \\
\hline \\
log(Duration)       &      --0.054\sym{***}&            &       0.003         &            &       0.006         &            &       0.019         &            &       0.019\sym{*}  \\
                    &     (0.015)         &            &     (0.015)         &            &     (0.015)         &            &     (0.015)         &            &     (0.011)         \\
[0.5em]
log(Amount)         &      --0.026\sym{***}&            &       0.016\sym{**} &            &      --0.016\sym{**} &            &       0.028\sym{***}&            &      --0.003         \\
                    &     (0.007)         &            &     (0.007)         &            &     (0.007)         &            &     (0.007)         &            &     (0.006)         \\
[0.5em]
\hline
Lasso method        &     plug--in         &            &     plug--in         &            &     plug--in         &            &     plug--in         &            &     plug--in         \\
$ N X$ var. sel.    &        8/64         &            &       12/64         &            &        5/64         &            &        4/64         &            &        7/64         \\
dep. var. mean      &        0.36         &            &        0.53         &            &        0.33         &            &        0.61         &            &        0.17         \\
$ N$ obs.           &       4,175         &            &       4,175         &            &       4,175         &            &       4,175         &            &       4,175         \\
\hline\hline
\end{tabular}
}


==> figtab/tab_grantstrat_all_lasso_interacts_s1_i0.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{10}{c}}
 \hline\hline
& & &  & \multicolumn{1}{c}{Larger} &  \\
& &\multicolumn{1}{c}{More} & \multicolumn{1}{c}{New}&\multicolumn{1}{c}{ongoing}&\multicolumn{1}{c}{More} \\
 &\multicolumn{1}{c}{Faster}&\multicolumn{1}{c}{risk}&\multicolumn{1}{c}{directions}&\multicolumn{1}{c}{projects}&\multicolumn{1}{c}{accurate}\\
\hline \\
log(Duration)       &       0.019\sym{*}  \\
                    &     (0.011)         \\
[0.5em]
\hspace{3mm} $\times$ Audience: Policymakers&       0.015         \\
                    &     (0.011)         \\
[0.5em]
log(Amount)         &      --0.003         \\
                    &     (0.006)         \\
[0.5em]
sizI*               &                     \\
                    &                     \\
[0.5em]
\hline
Incl. main effect   &           Y         \\
Lasso method        &     plug--in         \\
$ N X$ var. sel.    &        7/61         \\
dep. var. mean      &        0.17         \\
$ N$ obs.           &       4,175         \\
\hline\hline
\end{tabular}
}


==> figtab/tab_grantstrat_all_noimr.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{9}{c}}
 \hline\hline
& & & & & & &Larger & & \\
& &  &More & &New & &ongoing & &More \\
&Faster & &risk & &directions & &projects &  &accurate \\
                    &\multicolumn{1}{c}{(1)}         &            &\multicolumn{1}{c}{(2)}         &            &\multicolumn{1}{c}{(3)}         &            &\multicolumn{1}{c}{(4)}         &            &\multicolumn{1}{c}{(5)}         \\
\hline \\
log(Duration)       &      --0.055\sym{***}&            &       0.012         &            &       0.007         &            &       0.019         &            &       0.018         \\
                    &     (0.015)         &            &     (0.016)         &            &     (0.015)         &            &     (0.015)         &            &     (0.011)         \\
[0.5em]
log(Amount)         &      --0.025\sym{***}&            &       0.017\sym{**} &            &      --0.016\sym{**} &            &       0.026\sym{***}&            &      --0.003         \\
                    &     (0.007)         &            &     (0.007)         &            &     (0.007)         &            &     (0.007)         &            &     (0.006)         \\
[0.5em]
\hline
dep. var. mean      &        0.36         &            &        0.53         &            &        0.33         &            &        0.61         &            &        0.17         \\
$ N$ obs.           &       4,175         &            &       4,175         &            &       4,175         &            &       4,175         &            &       4,175         \\
\hline\hline
\end{tabular}
}


==> figtab/tab_indifhet_capintense_fundrprod.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{7}{c}}
\hline\hline
& \multicolumn{3}{c}{Capital intensity} & &\multicolumn{2}{c}{Fundraising productivity} \\ \cline{2-4} \cline{6-7}
            &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &            &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\hline
            &                     &                     &                     &            &                     &                     \\
$\gamma$    &       0.757\sym{***}&       0.754\sym{***}&       0.791\sym{***}&            &       0.804\sym{***}&       0.742\sym{***}\\
            &    (0.0126)         &    (0.0122)         &    (0.0115)         &            &    (0.0131)         &    (0.0142)         \\
[1em]
\hline
\\ m.r.s.   &      60,571         &      61,490         &      50,130         &            &      46,389         &      65,433         \\
\hspace{3mm} &     [7.7\%]         &     [7.9\%]         &     [6.4\%]         &            &     [5.9\%]         &     [8.4\%]         \\
[1em] \hline Sample&         Low         &         Mid         &        High         &            &         Low         &        High         \\
$ R^2$      &        0.85         &        0.86         &        0.90         &            &        0.92         &        0.85         \\
$ N$ obs.   &       1,392         &       1,393         &       1,390         &            &         963         &         934         \\
\hline\hline
\end{tabular}
}


==> figtab/tab_indifhet_discount.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\hline\hline
& \multicolumn{5}{c}{Age} \\ \cline{2-6}
            &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\hline
            &                     &                     &                     &                     &                     \\
$\gamma$    &       0.760\sym{***}&       0.752\sym{***}&       0.757\sym{***}&       0.808\sym{***}&       0.793\sym{***}\\
            &    (0.0137)         &    (0.0126)         &    (0.0146)         &    (0.0182)         &    (0.0256)         \\
[1em]
\hline
\\ m.r.s.   &      59,480         &      62,182         &      60,627         &      45,309         &      49,682         \\
\hspace{3mm} &     [7.6\%]         &     [8.0\%]         &     [7.8\%]         &     [5.8\%]         &     [6.4\%]         \\
[1em] \hline Age&       $<$35         &      36--45         &      46--55         &      56--65         &       $>$65         \\
$ R^2$      &        0.88         &        0.88         &        0.86         &        0.89         &        0.86         \\
$ N$ obs.   &         916         &       1,154         &         991         &         736         &         378         \\
\hline\hline
\end{tabular}
}


==> figtab/tab_indifhet_riskaver.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{8}{c}}
\hline\hline
& \multicolumn{3}{c}{Research risk-taking} & &\multicolumn{3}{c}{Personal risk-taking} \\ \cline{2-4} \cline{6-8}
            &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &            &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\hline
            &                     &                     &                     &            &                     &                     &                     \\
$\gamma$    &       0.740\sym{***}&       0.794\sym{***}&       0.771\sym{***}&            &       0.753\sym{***}&       0.776\sym{***}&       0.770\sym{***}\\
            &    (0.0119)         &    (0.0116)         &    (0.0125)         &            &    (0.0131)         &    (0.0104)         &    (0.0132)         \\
[1em]
\hline
\\ m.r.s.   &      65,861         &      49,398         &      56,181         &            &      61,826         &      54,768         &      56,579         \\
\hspace{3mm} &     [8.4\%]         &     [6.3\%]         &     [7.2\%]         &            &     [7.9\%]         &     [7.0\%]         &     [7.2\%]         \\
[1em] \hline Sample&         Low         &         Mid         &        High         &            &         Low         &         Mid         &        High         \\
$ R^2$      &        0.85         &        0.89         &        0.88         &            &        0.87         &        0.89         &        0.86         \\
$ N$ obs.   &       1,454         &       1,593         &       1,128         &            &       1,090         &       1,706         &       1,379         \\
\hline\hline
\end{tabular}
}


==> figtab/tab_stratpwcorr.tex <==
\begin{tabular}{l*{5}{c}}
\hline\hline
         
        &$ \uparrow$ speed&$ \uparrow$ risk& explore& exploit&$ \uparrow$ accuracy\\
\hline
$ \uparrow$ speed&   1&     &     &     &     \\
$ \uparrow$ risk&  --0.41&   1&     &     &     \\
explore     &  --0.31&  --0.08&   1&     &     \\
exploit     &  --0.16&  --0.33&  --0.41&   1&     \\
$ \uparrow$ accuracy&  --0.14&  --0.27&  --0.22&  --0.15&   1\\
\hline\hline
\end{tabular}


==> figtab/tab_stratpwmean.tex <==

\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\newcolumntype{L}{>{\raggedright\arraybackslash}X}
\newcolumntype{C}{>{\centering\arraybackslash}X}

\begin{tabular}{l r r r r r}

\hline
{}&{speedier}&{riskier}&{explore}&{exploit}&{accuracy} \tabularnewline
\hline
speedier&&&&& \tabularnewline
riskier&0.09&&&& \tabularnewline
explore&0.05&0.16&&& \tabularnewline
exploit&0.18&0.24&0.11&& \tabularnewline
accuracy&0.04&0.04&0.02&0.08& \tabularnewline
\hline 

\end{tabular}



==> figtab/tab_stratpwreg.tex <==

\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\newcolumntype{L}{>{\raggedright\arraybackslash}X}
\newcolumntype{C}{>{\centering\arraybackslash}X}

\begin{tabular}{l r r r r r}

\hline
{}&{speedier}&{riskier}&{explore}&{exploit}&{accuracy} \tabularnewline
\hline
speedier&&&&& \tabularnewline
riskier&--0.06&&&& \tabularnewline
explore&--0.27&1.16&&& \tabularnewline
exploit&1.07&0.95&0.09&& \tabularnewline
accuracy&0.36&--0.31&--0.51&0.62& \tabularnewline
\hline 

\end{tabular}


